A Subjective Interestingness measure for Business Intelligence explorations

This paper addresses the problem of defining a subjective interestingness measure for BI exploration. Such a measure involves prior modeling of the belief of the user. The complexity of this problem lies in the impossibility to ask the user about the degree of belief in each element composing their knowledge prior to the writing of a query. To this aim, we propose to automatically infer this user belief based on the user's past interactions over a data cube, the cube schema and other users past activities. We express the belief under the form of a probability distribution over all the query parts potentially accessible to the user, and use a random walk to learn this distribution. This belief is then used to define a first Subjective Interestingness measure over multidimensional queries. Experiments conducted on simulated and real explorations show how this new subjective interestingness measure relates to prototypical and real user behaviors, and that query parts offer a reasonable proxy to infer user belief.

==> main_algorithm.tex <==
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}
\caption{Evaluation algorithm}\label{algo:eval}
\algorithmicrequire A session $s$ to be evaluated (as an ordered list of queries), the global log $L$ and a database schema $D$\\
\algorithmicensure The subjective interestingness of each query of $s$
\begin{algorithmic}[1]

\State $G_t \gets $ BuildSchemaGraph(S) \Comment{see Algorithm \ref{algo:graph_building_schema}}
\State $G_l \gets $BuildLogGraph(L) \Comment{see Algorithm \ref{algo:graph_building}}
\State $G_{c} \gets MergeSchemaAndLogGraphs(G_t, G_l)$
\For{$i \in \llbracket 1, |s| \rrbracket $} \Comment{For each query in the session}
    \State $\textit{current\_session} \gets$ $[ s[j], j \in \llbracket 1, i \rrbracket ]$
    \State $\textit{current\_session\_graph} \gets InterconnectAll(\textit{current\_session})$
    \State $Gs_{t} \gets InterpolateNormalize(\textit{$G_c$},\textit{current\_session\_graph})$
    \State $belief \gets PageRank( Gs_t )$
    \State \textbf{Yield} $SubjectiveInterestingness(s[i], belief)$ \Comment{as described by Eq.  \ref{eq:si_sum}}
\EndFor

\Function{InterconnectAll}{L}
    \State $V \gets \emptyset$, $E \gets \emptyset $
    \For{$q \in L$}
        \State $V \gets V \cup parts(q)$
    \EndFor
    \For{$p_1 \in V$}
        \For{$p_2 \in V$}
            \State $E \gets E \cup \{ \tuple{p_1,p_2,1} \}$
        \EndFor
    \EndFor
    \Return $\tuple{V,E}$
\EndFunction
\end{algorithmic}
\end{algorithm}





==> tests_reco.tex <==
\section{How usage and recommendation impact belief}\label{sec:tests3}

The first experiments reported in Section \ref{sec:tests} show that our model of belief is able to transcribe different exploration templates based on the shape of their probability distribution functions, although $3$ templates, namely \textit{Explorative}, \textit{Goal Oriented} and \textit{Slice And Drill}, remain very close in this respect.

However, if our belief model is to be faithful to the user intent, as it is expressed at the query part level, any change in the accessed area of a cube should be traduced by a change in the assigned probability weights in our belief model. We propose to first simulate this diversity in the cube exploration by learning the belief model on different and independent log files generated by CubeLoad.

Second, as the long-term objective is to use belief-based interestingness measure as an input for tailoring personalized recommendations, we want to evaluate to which extent the output of a recommender system could impact the belief of a specific user. To this aim, we use a state-of-the-art OLAP recommender system \cite{DBLP:journals/dss/AligonGGMR15} that is trained on a log file representative of a specific CubeLoad template and whose output recommendation is used to define a new belief distribution. It is important to notice that, at this step, we consider that all recommended queries are executed at the same time and that the belief can be computed based on the same prior knowledge from the user for all recommended queries at once. As explained earlier, dealing with the evolution of the user belief after each query is out of the scope of this paper.

% Then, in order to evaluate to which extent a recommender system and the usage (i.e. the log used to build the model) impacts our belief model
In both cases, we need to define beforehand a \textit{reference belief}  for each of the $4$ CubeLoad templates in our simulations. Then a divergence measure can traditionally be used to evaluate to which extent changing the template or changing the log file on which we learn the models impacts the belief distribution.

\subsection{Experimental protocol}

\paragraph{Evaluation scenarios} Figure \ref{fig:protocol} presents the main evaluation protocol for the impact of usage and recommender system on the belief measure. The left-side of Figure \ref{fig:protocol} illustrates how to generate the \textit{reference belief}. Similarly to Section \ref{sec:xp_protocol}, we use $50$ CubeLoad sessions among which $43$ are used to compute the topology graph of our PageRank (see \textit{``Log usage construction rules''} in Section \ref{sec:PRbelief}) and $7$ sessions issued from a single CubeLoad template are used to simulate a user and bias the topic-specific PageRank. 

The right-side of Figure \ref{fig:protocol} describes how we generate the \textit{test belief} based on the  recommender system \cite{DBLP:journals/dss/AligonGGMR15} and a simulated user of the recommender system. To do so, we generate a new \textit{independent} log file from which $10$ random sessions from a single CubeLoad template are drawn. They are used to train the recommender system. In addition a separate session is drawn and truncated to be used as a seed for the recommender. In order to evaluate to which extent the diversity of queries affects our belief model, we also consider the case where the recommender system as well as the seed session for the recommender are drawn at random from the same log file as the one used for the reference belief. We call this scenario \textit{identical} while the first one with distinct session files is named \textit{independent} hereafter.

%identical We propose two scenarios to evaluate the impact of usage and recommendation on belief: either the test log file is \textit{independent} from the \textit{reference} log file or it is set \textit{identical}. In case where the log file is \textit{independent}, it contains $160$ sessions, with $40$ sessions per CubeLoad template.


\begin{figure*}
    \begin{center}
    \includegraphics[scale=0.5]{img/experimental_protocol.png}
    \caption{Evaluation protocol for the impact of usage and recommender system on the belief measure.}
    \label{fig:protocol}
    \end{center}
\end{figure*}

\paragraph{Evaluation of results} 
%For the sake of clarity, we 
We use the Hellinger distance as described in Section \ref{sec:xp_protocol} to compare the reference and test belief distributions.
We generate 40 random logs (10 per profile) %from a pool of 200 
and we run them against randomly chosen seeds from the 4 profiles and against the 4 possible reference belief models. Results are    %\nico{@Alex: check how we perform cross-validation.} We run each comparison between a reference profile and a random recommender test 10 times for each configuration 
averaged 
and reported 
%(and standard deviation although not reported here) Hellinger distance values 
in Table \ref{tab:identical} and \ref{tab:independent}.

%\alex{@Nicolas, j'ai mis la cross validation tel qu'on l'a implementé}
%\nico{ok, j'ai enleve le from a pool of 200 qui complique la lecture a mon avis.}
% Part with Jensen-Shannon divergence description
%Probabilistic measures are traditionally compared with a divergence measure rather than a distance like Euclidean or Mahalanobis distances. Indeed, distances requires that symmetry and triangular inequality are respected. In our case, we only need symmetry and for this reason we propose to use the well-known Jensen-Shannon divergence which is a symmetric extension of the Kullback-Leibler divergence. For two probability distributions $P$ and $Q$ defined over the same probability space, the Jensen-Shannon divergence $JSD(P,Q)$ is defined as follows:
%\begin{equation}
%    JSD(P,Q)=JSD(Q,P)=\frac{1}{2} KL(P,M) + \frac{1}{2} KL(Q,M)
%\end{equation}
%where $M = \frac{1}{2}(P+Q)$ is the average probability distribution and $KL(P,M)$ denotes the Kullback-Leibler divergence between two probability distribution $P$ and $M$ as follows:
%\begin{equation}
%    KL(P,M)=\sum_{i} P(i)\times \log \left( \frac{M(i)}{P(i)} \right)
%\end{equation}
% It is important to notice that in our case, because we use a topic-specific PageRank algorithm it is impossible to end up with a probability equal to $0$. Therefore, the Jensen-Shannon divergence is always defined.

% Part with Kullback-Leibler description
%In our case, we have a reference probability distribution and a test distribution, so we propose to use the Kullback-Leibler divergence. For two probability distributions, a reference $P$ and a test $Q$ defined over the same probability space, the Kullback-Leibler divergence $KL(P||Q)$ is defined as follows:
%\begin{equation}
%    KL(P||Q)=\sum_{i} P(i)\times \log \left( \frac{Q(i)}{P(i)} \right)
%\end{equation}
%It is important to notice that in our case, because we use a topic-specific PageRank algorithm it is impossible to end up with a probability equal to $0$ in the reference probability $P$. Therefore, the Kullback-Leibler divergence is always defined.

%*********
\subsection{Hypothesis}

We expect several observable results from these experiments. First, it is expected that the belief divergence between the recommended queries from the \textit{test} and the queries used as a \textit{re\-fe\-ren\-ce} is much larger in case of \textit{in\-de\-pen\-dent} log files than in case of \textit{identical} log files. As in both cases the recommender system is involved, this would mean that any observed difference would be due to the difference in log files and that our belief model while preserving the distribution probabilities of each CubeLoad template is able to reflect the differences in usage on query parts.

Second, we expect to observe differences between the $4$ CubeLoad templates that  could refine the observations of Section \ref{sec:53}. Indeed, only based on the distribution it was not possible in our setting to distinguish clearly among the \textit{Explorative}, \textit{Goal Oriented} and \textit{Slice and Drill} templates. We expect them to remain close but with slight divergence that would reflect the different abilities of each template to dig into new parts of the data cube. However, similarly to experiments in Section \ref{sec:53} we expect \textit{Slice All} to be significantly divergent from the other profiles. Indeed, it is known that this template exhibits tendencies to explore locally the cube by only navigating a dimension following siblings relations. 


Finally, if we consider our belief model as representative of the usage, we may be able to draw conclusions about the use of recommender systems with CubeLoad templates and to which extent the latter propose really distinguishable exploration patterns. To this aim, a comparison of divergence values when comparing, for each CubeLoad template, its reference to its recommended test on the same log file would indicate to which extent the template explores various portion of the cube. In other words, the more explorative a template is, the larger the divergence between a recommendation based on this template and its reference should be.

%Finally, we can also study to which extent a test on a template is close to the reference from the same template when evaluated on the same log (scenario \textit{identical}). In this context, we expect 
%
%itself as an explorative profile, and even more a recommendation based on it, will have tendencies to propose new query parts that are unlikely while a \textit{Slice All} profile may have a tendency to cycle around the same concepts and trap a user in a cognitive bubble.

%*********
\subsection{Results}

% Intro
Tables \ref{tab:identical} and \ref{tab:independent} present experimental values of Hellinger distance %Kullback-Leibler 
for the \textit{identical} and the \textit{independent} scenarios and each type of recommendation based on the $4$ CubeLoad templates (lines) for each reference belief model (columns).

It can be seen that, as expected, the divergence is significantly lower when considering recommendations based on the same log file that was used for the reference belief computation. This shows that our belief method is sensitive to the actual queries that are involved in the building of the model despite the general trends observed for the probability distribution in Section \ref{sec:53}.

\begin{table}[ht]
\footnotesize
\begin{center}
\begin{tabular}{lcccc} \hline
Tests$\backslash$References & \textit{Explorative}	& \textit{Goal Oriented} & \textit{Slice All} & \textit{Slice and Drill} \\ \hline
% Kullback-Leibler
%\textit{Explorative} & \textbf{1.68} & 1.50 & 1.05 & 1.55 \\
%\textit{Goal Oriented} & 1.75 & \textbf{1.39} & 0.82 & 1.50 \\
%\textit{Slice All} & 1.99 & 1.89 & \textbf{1.02} & 1.83 \\
%\textit{Slice and Drill} & 1.67 & 1.32 & 0.85 & \textbf{1.42} \\ \hline
% Jensen-Shannon
%\textit{Explorative} & \textbf{0.47} & 0.42 & 0.31 & 0,42 \\
%\textit{Goal Oriented} & 0.48 & \textbf{0.40} & 0.24 & 0,41 \\
%\textit{Slice All} & 0,52 & 0.49 & \textbf{0.28} & 0,47 \\
%\textit{Slice and Drill} & 0.47 & 0.37 & 0.25 & \textbf{0,40} \\  \hline
% Hellinger
\textit{Explorative} & \textbf{0.64} & 0.60 & 0.47 & 0.60 \\
\textit{Goal Oriented} & 0.64 & \textbf{0.61} & 0.46 & 0.60 \\
\textit{Slice All} & 0.67 & 0.63 & \textbf{0.47} & 0.62 \\
\textit{Slice and Drill} & 0.63 & 0.60 & 0.43 & \textbf{0.58} \\ \hline
\end{tabular}
\caption{%Kullback-Leibler 
%Jensen-Shannon 
Average Hellinger distance values on 10 runs when log files are \textbf{identical}. Lines represent test and columns represents reference belief.}
\label{tab:identical}
\end{center}
\end{table}

\begin{table}[ht]
\begin{center}
\footnotesize
\begin{tabular}{lcccc} \hline
Tests$\backslash$References & \textit{Explorative} & \textit{Goal Oriented} & \textit{Slice All} & \textit{Slice and Drill} \\ \hline
% Kullback-Leibler
%\textit{Explorative} & \textbf{1.15} & 1.20 & 0.95 & 1.33 \\
%\textit{Goal Oriented} & 1.14 & \textbf{1.15} & 0.90 & 1.25 \\
%\textit{Slice All} & 2.38 & 2.41 & \textbf{2.19} & 2.54 \\
%\textit{Slice and Drill} & 0.83 & 0.85 & 0.66 & \textbf{0.90} \\ \hline
% Jensen-Shannon
%\textit{Explorative} & \textbf{0.78} & 0.80 & 0.73 & 0.81 \\
%\textit{Goal Oriented} & 0.79 & \textbf{0.79} & 0.73 & 0.81 \\
%\textit{Slice All} & 0.76 & 0.76 & \textbf{0.71} & 0.78 \\
%\textit{Slice and Drill} & 0.79 & 0.80 & 0.75 & \textbf{0.81} \\ \hline
% Hellinger
\textit{Explorative} & 0.85 & 0.86 & 0.81 & 0.86 \\
\textit{Goal Oriented} & 0.85 & 0.85 & 0.81 & 0.86 \\
\textit{Slice All} & 0.83 & 0.84 & 0.79 & 0.84 \\
\textit{Slice and Drill} & 0.86 & 0.86 & 0.82 & 0.87 \\ \hline
\end{tabular}
\caption{%Kullback-Leibler 
% Jensen-Shannon 
Average Hellinger distance values on 10 runs when log files are \textbf{independent}. Lines represent test and columns represents reference belief.}
\label{tab:independent}
\end{center}
\end{table}


Then, results from Tables \ref{tab:identical} and \ref{tab:independent} corroborates that there exists differences between the CubeLoad templates but that are more or less difficult to observe depending on the CubeLoad template, as shown by the distribution of Section \ref{sec:53}.

In the identical scenario, \textit{Explorative} recommendation is the most distant to its corresponding \textit{Explorative} reference (distance $= 0.64$) and the most distant to all other recommendations as shown in column \textit{Explorative} from Table \ref{tab:identical}. This %may be explained 
can be understood
by the nature of the CubeLoad template which makes it difficult to model for a recommender system, which in turns implies a higher probability to access new portions of the cube and thus new query parts.

\textit{Goal oriented} column of Tables \ref{tab:identical} and \ref{tab:independent} presents not significantly different distance values whatever the recommendation profile is. This is expected as this template can generate several different paths in the cube to access the same region in the end. As a consequence, there is a variety in the accessed query parts which in turns tends to smooth the distance values.

\textit{Slice and Drill} exhibits significant differences and with a small distance to itself of $0.58$, which means that the recommendation that is produced reflects the CubeLoad template and stays in a localized region of the data cube with more common query parts between recommendations and the reference template.

% this is no more true!
%\it can be observed in both scenarios that the distances between all CubeLoad templates but \textit{Slice All} are not significantly different even if some minor changes can be noticed (standard deviation are not reported here but have been studied). 

%That corroborates that there exists differences between the CubeLoad templates but that are difficult to observe as shown by the distribution of Section \ref{sec:53}. A more thoroughful analysis of these results is needed to conclude and is left as future work.\\

%However, if we consider only the diagonal values of Table \ref{tab:identical}, where the log file is the same between test and reference, it is possible to observe that the \textit{Explorative} template has a higher ``inner'' divergence (between its reference and test belief) of $0.64$ than the other profiles. This may be explained by its explorative nature, as the name suggest, which implies a higher probability to access new portions of the cube and thus new query parts. However, it should be noted that all tests recommendations tends to be more distant to the \textit{Explorative} reference while it is more difficult to conclude about \textit{Goal Oriented} with distances to all test templates not significantly different mainly due to a larger standard deviation. \textit{Slice and Drill} exhibits significant differences and with a small distance to itself of $0.58$, which means that the recommendation that is produced reflects the CubeLoad template and stays in a localized region of the data cube with more common query parts between recommendations and the reference template.\\

Finally, an interesting observation is that \textit{Slice All} has a very low inner distance of $0.47$ in Table \ref{tab:identical} which means that the exploration is very focused and that even a recommender system based on this template will reproduce this local exploration behaviour with no surprising query parts. This reflects a sort of cognitive bubble associated to this template, which can be detected with our approach of user belief estimation. 

The latter is confirmed by the analysis of the line \textit{Slice All} in Table \ref{tab:identical} where the distance between the recommended \textit{Slice All} and the other CubeLoad reference templates that are higher than the other distances for each of these templates. For example, in Table \ref{tab:identical}, the distance of \textit{Slice All} to \textit{Explorative} is $0.67$ which is the largest distance for the column \textit{Explorative}.\\

These first results bring new insights on our belief model, and to which extent it is coherent with the CubeLoad profiles. A more thoroughful analysis of these results is needed to conclude about differences on CubeLoad templates and is left as future work.

% Old versions
%It is interesting to notice that in the case of identical log files, \textit{Slice All} is significantly different from the other template when considering its line in Table \ref{tab:identical}. This again corroborates observed difference in terms of probability distribution with a difference in which query part is queried most by this profile. 

% analysis of Slice All ==> go to possible cognitive bubble?
%In the case of \textit{identical} log files \textit{Slice All} test is supposed to have a greater divergence with the other reference templates than divergences when compared to the case of \textit{independent} log files. Indeed, in the case of \textit{identical} log files, as the exploration space is more limited than in the case of \textit{independent} log files, the local search behaviour of \textit{Slice All} is even more noticeable while the other templates that explores more the unique log files have more chances to query the same part of the cube.
%in terms of produced divergence measures when compared while the difference with the  should be more pronounced. 

==> trash.tex <==
\subsubsection{DOPAN use case}


\begin{figure}[h]
    \centering
    \includegraphics[scale=0.24]{dopan_results/box_plot_SI_skill_and_user.png}
    \caption{Exploration Subjective Interestingness by skill level for users exploring the DOPAN cubes \patrick{preciser que c'est par exploration et pas par user}}
    \label{fig:dopan_box_plot}
\end{figure}

From Figure \ref{fig:dopan_box_plot} we can observe that the explorations tagged with the lowest skill levels yield the most subjective information, which is expected because of the user weaker knowledge of the cubes. Indeed, if the user explores a larger part of the cubes, by construction, the probability of knowing the query parts attached to these portions of the cube increase and so the surprise and SI attached to these query decreases. This has been confirmed by a careful study of the logs where for some users, such as Student 4 whose skill went from ``B'' to ``D'' in the course of $5$ sessions over a few days. Overall only $2$ students were able to perform a session rated ``D'' (best score) on their first try and thus most users with ``D'' explorations will have already explored the cubes at least a few times. 
\patrick{toujours pas clair pour moi}


Interestingly, explorations with lower score (``B'') are not necessarily the shortest explorations in terms of number of queries. As a consequence, the observed difference in scores can mainly be explained by differences in the exploration pattern.

%as their knowledge of the cube expends (by making more sessions) the skill level of their explorations increase. this particularly true for

%\patrick{est-ce que ce ne serait pas plutot que les mauvaises sessions ont un comportement plus exploratoire, a la slice and drill, sans etre concentrées sur un probleme (inverse du slice all finalement).}
%\alex{[Reponse pour @Patrick] 
Analysis by an expert of all "B" skill sessions reveals a few insights. First, most sessions start with 10 or more near identical or identical queries where the user only changes {\it measures}, then users will try to change the {\it group by set} (one element at a time). Finally, at mid sessions,  users will start changing {\it Group by set} elements combined with {\it selection} predicates (very simple, one or two dimensions at most). This behavior looks similar to the Slice and Drill pattern described on Figure \ref{fig:template} although noisier and more erratic at times.%}
%Skype ????
%Aussi, les mauvaises sessions sont sans doute les plus courtes (a verifier) et il se trouve que les slice and drill sont aussi les plus courtes, est-ce une coincidence ?}

%\nico{non les sessions les plus mauvaises ne sont pas les plus courtes}

%\patrick{pas sur, tous les utilisateurs avaient la meme connaissance du cube a priori} 

As shown in Figure \ref{fig:dopan_box_plot}, the exploration Subjective Interestingness measure fails to fully discriminate between the medium and advanced users. 
%This could indicate that the greater skill level ``D'' manages to obtain highly subjectively interesting patterns part of the time. At the contrary, the ``C'' skill has sessions that are less interesting with lower variation, indicating that their knowledge of the cube has improved but they still have trouble to find new interesting patterns.}


\patrick{il faudrait aussi analyser les 2 composantes de SI : le belief et le nombre de query parts}

To highlight the differences implied by the SI between the true skills, Figure \ref{fig:dopan_violin} shows the distributions of the measure at the query level (and not by exploration) for each skill category, with the actual sample in white 
\patrick{preciser: comment sont ordonnes les samples}
as a KDE estimate alone can hide subtle details.  
%This time, the queries SI are directly aggregated by skill to show the results as three distributions.

\begin{figure}[ht]
    \centering
    \hspace{-1.5cm}
    \includegraphics[scale=0.38]{dopan_results/violin_plot_SI_skills.png}
    \caption{Distributions of the query Subjective Interestingness by user skill level}
    \label{fig:dopan_violin}
\end{figure}

It is directly apparent that the distributions have different shapes in accordance to the skill level. The skewness of the distributions are very different (-0.68 for B 1.32 for C and 0.46 for D). Between ``B'' and ``C'', there is a great shift in skewness, from negative to positive. This can be explained by the fact that the user are gaining more knowledge of the cube as well as improving their exploration skills. A less skilled user will very easily find interesting patterns because of his limited knowledge of the cube at the beginning. This explain the negative skew of the distribution. For the second skill level, ``C'', their exploration skills are still improving. As they fail to find new interesting data with their exploration method, this effectively skews the distribution toward lower SI. Finally, the ``D'' skill levels shows two modes which seem to be the merging of the two previous behaviors. The lower mode is made of the queries who produced the least amount of interestingness because of the previous user's knowledge of the cube. The higher mode emphasize the fact that a skilled user will still find new ways to explore the cube, though generating a greater amount of Subjective Interestingness. 

Moreover, it is important to notice that using the query results or any data from cube were not needed to observe this differences and only depends on the sequences of query parts used in the explorations. This observation legitimates our choice of using the sole query parts as a proxy for the values of cells. %which consisted in not using the query result data to compute the Subjective Interestingness.


